D$^2$CSG: Unsupervised Learning of Compact CSG Trees with Dual Complements and Dropouts

We present D$^2$CSG, a neural model composed of two dual and complementary network branches, with dropouts, for unsupervised learning of compact constructive solid geometry (CSG) representations of 3D CAD shapes. Our network is trained to reconstruct a 3D shape by a fixed-order assembly of quadric primitives, with both branches producing a union of primitive intersections or inverses. A key difference between D$^2$CSG and all prior neural CSG models is its dedicated residual branch to assemble the potentially complex shape complement, which is subtracted from an overall shape modeled by the cover branch. With the shape complements, our network is provably general, while the weight dropout further improves compactness of the CSG tree by removing redundant primitives. We demonstrate both quantitatively and qualitatively that D$^2$CSG produces compact CSG reconstructions with superior quality and more natural primitives than all existing alternatives, especially over complex and high-genus CAD shapes.

==> tables/mesh2csg_shapenet.tex <==
\begin{table}[t!]
\centering
%  \caption{Comparing CSG representation learning from 3D meshes in ShapeNet.}
  \caption{Comparing CSG rep learning from meshes in ShapeNet.}
 
 %UCSG and CSG-Stump do not produce surface primitives, only boxes and spheres, which are convex --- we count them only under convexes.
 
\label{tab:mesh2csg_shapenet}

 \begin{tabular}{l r r r r}

    % \toprule
     \hline
 Methods & BSP & STUMP & CAPRI & Ours\\
    % \midrule
    %     \addlinespace[5pt]
    \hline
CD $\downarrow$                 & 0.164   & 2.214   & 0.124  & \textbf{0.119} \\
NC $\uparrow$                   & 0.882   & 0.794   & \textbf{0.890}  & 0.887 \\
ECD $\downarrow$                & 3.899  & 6.101   & 2.035 & \textbf{1.722}\\
LFD $\downarrow$                & 2135.68  & 4267.66      & 1558.08  & \textbf{1506.13} \\
\#P $\downarrow$ & 694.21  & 228.58  & \textbf{50.94}      & 63.78 \\
%\#Intersections (\#C) $\downarrow$ & 78.43  & 84.32  &  \textbf{8.33}     & 11.06 \\
  % \bottomrule
  \hline
\end{tabular}

\end{table}

==> tables/notrain.tex <==
\begin{table}[t!]
\centering
  \caption{Comparing methods under the same auto-decoder setting.}
 
 %UCSG and CSG-Stump do not produce surface primitives, only boxes and spheres, which are convex --- we count them only under convexes.
 
\label{tab:notrain}

 \begin{tabular}{l r r |r r }

    % \toprule
     \hline
     & \multicolumn{2}{c}{ABC} & \multicolumn{2}{c}{ShapeNet} \\
     \hline
 Methods & CAPRI & Ours & CAPRI & Ours\\
    % \midrule
    %     \addlinespace[5pt]
    \hline
CD $\downarrow$                 & 0.183   & \textbf{0.071}   & 0.156 & \textbf{0.119} \\
NC $\uparrow$                   & 0.907   & \textbf{0.928}   & 0.882 & \textbf{0.887} \\
ECD $\downarrow$                & 3.918  & \textbf{3.467}   & 2.359 & \textbf{1.722}\\
LFD $\downarrow$                & 635.01  & \textbf{490.48} & 1685.38   & \textbf{1506.13} \\
\#P $\downarrow$ & 77.15  & \textbf{58.81}  & \textbf{52.13} & 63.78 \\
%\#Intersections (\#C) $\downarrow$ & 28.38  & 13.43      &  \textbf{8.31}     & 8.87 \\
  % \bottomrule
  \hline
\end{tabular}

\end{table}
